Deep Convolutional Neural Networks for Breast Cancer Histology Image Analysis

Breast cancer is one of the main causes of cancer death worldwide. Early diagnostics significantly increases the chances of correct treatment and survival, but this process is tedious and often leads to a disagreement between pathologists. Computer-aided diagnosis systems showed potential for improving the diagnostic accuracy. In this work, we develop the computational approach based on deep convolution neural networks for breast cancer histology image classification. Hematoxylin and eosin stained breast histology microscopy image dataset is provided as a part of the ICIAR 2018 Grand Challenge on Breast Cancer Histology Images. Our approach utilizes several deep neural network architectures and gradient boosted trees classifier. For 4-class classification task, we report 87.2% accuracy. For 2-class classification task to detect carcinomas we report 93.8% accuracy, AUC 97.3%, and sensitivity/specificity 96.5/88.0% at the high-sensitivity operating point. To our knowledge, this approach outperforms other common methods in automated histopathological image classification. The source code for our approach is made publicly available at https://github.com/alexander-rakhlin/ICIAR2018

==> gradlew <==
#!/usr/bin/env bash

##############################################################################
##
##  Gradle start up script for UN*X
##
##############################################################################

# Attempt to set APP_HOME
# Resolve links: $0 may be a link
PRG="$0"
# Need this for relative symlinks.
while [ -h "$PRG" ] ; do
    ls=`ls -ld "$PRG"`
    link=`expr "$ls" : '.*-> \(.*\)$'`
    if expr "$link" : '/.*' > /dev/null; then
        PRG="$link"
    else
        PRG=`dirname "$PRG"`"/$link"
    fi
done
SAVED="`pwd`"
cd "`dirname \"$PRG\"`/" >/dev/null
APP_HOME="`pwd -P`"
cd "$SAVED" >/dev/null

APP_NAME="Gradle"
APP_BASE_NAME=`basename "$0"`

# Add default JVM options here. You can also use JAVA_OPTS and GRADLE_OPTS to pass JVM options to this script.
DEFAULT_JVM_OPTS=""

# Use the maximum available, or set MAX_FD != -1 to use that value.
MAX_FD="maximum"

warn ( ) {
    echo "$*"
}

die ( ) {
    echo
    echo "$*"
    echo
    exit 1
}

# OS specific support (must be 'true' or 'false').
cygwin=false
msys=false
darwin=false
nonstop=false
case "`uname`" in
  CYGWIN* )
    cygwin=true
    ;;
  Darwin* )
    darwin=true
    ;;
  MINGW* )
    msys=true
    ;;
  NONSTOP* )
    nonstop=true
    ;;
esac

CLASSPATH=$APP_HOME/gradle/wrapper/gradle-wrapper.jar

# Determine the Java command to use to start the JVM.
if [ -n "$JAVA_HOME" ] ; then
    if [ -x "$JAVA_HOME/jre/sh/java" ] ; then
        # IBM's JDK on AIX uses strange locations for the executables
        JAVACMD="$JAVA_HOME/jre/sh/java"
    else
        JAVACMD="$JAVA_HOME/bin/java"
    fi
    if [ ! -x "$JAVACMD" ] ; then
        die "ERROR: JAVA_HOME is set to an invalid directory: $JAVA_HOME

Please set the JAVA_HOME variable in your environment to match the
location of your Java installation."
    fi
else
    JAVACMD="java"
    which java >/dev/null 2>&1 || die "ERROR: JAVA_HOME is not set and no 'java' command could be found in your PATH.

Please set the JAVA_HOME variable in your environment to match the
location of your Java installation."
fi

# Increase the maximum file descriptors if we can.
if [ "$cygwin" = "false" -a "$darwin" = "false" -a "$nonstop" = "false" ] ; then
    MAX_FD_LIMIT=`ulimit -H -n`
    if [ $? -eq 0 ] ; then
        if [ "$MAX_FD" = "maximum" -o "$MAX_FD" = "max" ] ; then
            MAX_FD="$MAX_FD_LIMIT"
        fi
        ulimit -n $MAX_FD
        if [ $? -ne 0 ] ; then
            warn "Could not set maximum file descriptor limit: $MAX_FD"
        fi
    else
        warn "Could not query maximum file descriptor limit: $MAX_FD_LIMIT"
    fi
fi

# For Darwin, add options to specify how the application appears in the dock
if $darwin; then
    GRADLE_OPTS="$GRADLE_OPTS \"-Xdock:name=$APP_NAME\" \"-Xdock:icon=$APP_HOME/media/gradle.icns\""
fi

# For Cygwin, switch paths to Windows format before running java
if $cygwin ; then
    APP_HOME=`cygpath --path --mixed "$APP_HOME"`
    CLASSPATH=`cygpath --path --mixed "$CLASSPATH"`
    JAVACMD=`cygpath --unix "$JAVACMD"`

    # We build the pattern for arguments to be converted via cygpath
    ROOTDIRSRAW=`find -L / -maxdepth 1 -mindepth 1 -type d 2>/dev/null`
    SEP=""
    for dir in $ROOTDIRSRAW ; do
        ROOTDIRS="$ROOTDIRS$SEP$dir"
        SEP="|"
    done
    OURCYGPATTERN="(^($ROOTDIRS))"
    # Add a user-defined pattern to the cygpath arguments
    if [ "$GRADLE_CYGPATTERN" != "" ] ; then
        OURCYGPATTERN="$OURCYGPATTERN|($GRADLE_CYGPATTERN)"
    fi
    # Now convert the arguments - kludge to limit ourselves to /bin/sh
    i=0
    for arg in "$@" ; do
        CHECK=`echo "$arg"|egrep -c "$OURCYGPATTERN" -`
        CHECK2=`echo "$arg"|egrep -c "^-"`                                 ### Determine if an option

        if [ $CHECK -ne 0 ] && [ $CHECK2 -eq 0 ] ; then                    ### Added a condition
            eval `echo args$i`=`cygpath --path --ignore --mixed "$arg"`
        else
            eval `echo args$i`="\"$arg\""
        fi
        i=$((i+1))
    done
    case $i in
        (0) set -- ;;
        (1) set -- "$args0" ;;
        (2) set -- "$args0" "$args1" ;;
        (3) set -- "$args0" "$args1" "$args2" ;;
        (4) set -- "$args0" "$args1" "$args2" "$args3" ;;
        (5) set -- "$args0" "$args1" "$args2" "$args3" "$args4" ;;
        (6) set -- "$args0" "$args1" "$args2" "$args3" "$args4" "$args5" ;;
        (7) set -- "$args0" "$args1" "$args2" "$args3" "$args4" "$args5" "$args6" ;;
        (8) set -- "$args0" "$args1" "$args2" "$args3" "$args4" "$args5" "$args6" "$args7" ;;
        (9) set -- "$args0" "$args1" "$args2" "$args3" "$args4" "$args5" "$args6" "$args7" "$args8" ;;
    esac
fi

# Split up the JVM_OPTS And GRADLE_OPTS values into an array, following the shell quoting and substitution rules
function splitJvmOpts() {
    JVM_OPTS=("$@")
}
eval splitJvmOpts $DEFAULT_JVM_OPTS $JAVA_OPTS $GRADLE_OPTS
JVM_OPTS[${#JVM_OPTS[*]}]="-Dorg.gradle.appname=$APP_BASE_NAME"

exec "$JAVACMD" "${JVM_OPTS[@]}" -classpath "$CLASSPATH" org.gradle.wrapper.GradleWrapperMain "$@"

